Revisiting Chase Termination for Existential Rules and their Extension to Nonmonotonic Negation

Existential rules have been proposed for representing ontological knowledge, specifically in the context of Ontology- Based Data Access. Entailment with existential rules is undecidable. We focus in this paper on conditions that ensure the termination of a breadth-first forward chaining algorithm known as the chase. Several variants of the chase have been proposed. In the first part of this paper, we propose a new tool that allows to extend existing acyclicity conditions ensuring chase termination, while keeping good complexity properties. In the second part, we study the extension to existential rules with nonmonotonic negation under stable model semantics, discuss the relevancy of the chase variants for these rules and further extend acyclicity results obtained in the positive case.

==> algos/propagation.tex <==
% algos/propagation.tex

\begin{algorithm}[ht!]
\DontPrintSemicolon
\caption{Propagation}
\label{alg:propagation}

\KwData{$Y$ : an initial set of variables, $WillPropagate$ : $(\{0,1\}^*,V) \rightarrow \{0,1\}$ a function
determining whether the marking procedure will propagate to an element of $V$}
\KwResult{}

%$Y \leftarrow \{y :$ y is an existentially quantified variable$\}$\;
$F \leftarrow \Gamma^+(Y)$\;
mark all terms in $F$\;

\While{$F \neq \emptyset$}{
	$x \leftarrow pop(F)$\;
	\For{$v \in \Gamma^+(x)$}{
		\If{$v$ is not marked and $WillPropagate(marked,v)$}{
%		\If{$(x,v)$ is a $special$-$edge$}{
%			\If{$WillPropagate(marked,v)$}{
%			%\If{$\forall t$ st $\exists (t,v), \forall$ position $\predpos{p}{i} \in Pos(t)$,
%			%$\exists a : \vxpg{t}{p}{i}{a}$ is marked}{
%				mark $v$\;
%				$F \leftarrow F \cup \{v\}$
%			}
%		}
%		\Else{
			mark $v$\;
			$F \leftarrow F \cup \{v\}$
		}
	}
}

\end{algorithm}



==> meta/dependencies-graph-old.tex <==
% meta/dependencies-graph.tex

%% some functions, and tikzstyles for drawing
%% gp, grd and gerd


%%%%% GERD

\newcounter{gerdRuleID}
\newcounter{gerdTermID}
\newcounter{gerdUnifID}
\newcounter{gerdNbBodyTerms}
\newcounter{gerdNbHeadTerms}

\newenvironment{gerd:figure}{
	\setcounter{gerdRuleID}{0}
	\setcounter{gerdUnifID}{0}
	\begin{tikzpicture}
}{
	\end{tikzpicture}
}

\tikzstyle{gerd:node}=[
]


\tikzstyle{gerd:fake}=[
	gerd:node,
	inner sep=0mm
	%circle,
	%draw=black
]

\tikzstyle{gerd:term}=[
	gerd:node,
	circle,
	minimum size=1mm,
	%draw=black,
	inner sep=0mm,
	draw=none
]

\tikzstyle{gerd:edge}=[
	->,
	draw=black
]

\tikzstyle{gerd:edge-norm}=[
	gerd:edge,
	%draw=blue!50!black
]

\tikzstyle{gerd:edge-spec}=[
	gerd:edge-norm
%	gerd:edge,
%	thick,
%	densely dotted,
%	draw=red!50!black
]

\tikzstyle{gerd:edge-unif}=[
	gerd:edge,
	%draw=green!50!black,
	%dashed,
	%thick
]

\tikzstyle{gerd:border}=[
	-,
	draw=black
]

\tikzstyle{gerd:border-ext}=[
	gerd:border,
	thick
]

\tikzstyle{gerd:border-int}=[
	gerd:border,
	draw=black!50!white,
	dashed
]


%%%
%% WARNING/ the reversse mode does not work anymore
%% should let the west/east variable

% 0: [1|0] reverse mode
% 1: X
% 2: Y
% 3: Xmax
% 4: Ymax
% 5: list of body terms
% 6: list of head terms
% 7: list of fr terms
% 8: list of exist terms
\newcommand{\gerdRule}[9][0]{
	\refstepcounter{gerdRuleID}

	% preprocessing
	\setcounter{gerdNbBodyTerms}{0}
	\setcounter{gerdNbHeadTerms}{0}
	\foreach \tb in {#6} { \refstepcounter{gerdNbBodyTerms} }
	\foreach \th in {#7} { \refstepcounter{gerdNbHeadTerms} }

	% fake nodes
	\foreach \i [evaluate=\i as \x using (((#4-#2)/4)*\i)+#2] in {0, 1, 2, 3, 4} {
		\node[gerd:fake] (fakeT\thegerdRuleID_\i) at (\x,#3) {};
	}
	\foreach \i [evaluate=\i as \x using (((#4-#2)/4)*\i)+#2, evaluate=\i as \y using #3+#3-#5] in {0, 1, 2, 3, 4} {
		\node[gerd:fake] (fakeB\thegerdRuleID_\i) at (\x,\y) {};
	}

	% draw borders
	\draw[gerd:border-ext] (fakeT\thegerdRuleID_0.center) -- (fakeT\thegerdRuleID_4.center)
						-- (fakeB\thegerdRuleID_4.center) -- (fakeB\thegerdRuleID_0.center)
						-- (fakeT\thegerdRuleID_0.center);
	\draw[gerd:border-int] (fakeT\thegerdRuleID_2.center) -- (fakeB\thegerdRuleID_2.center);


	% compute body terms
	\ifthenelse{\equal{#1}{1}}{
		\pgfmathparse{#2+(3*((#4-#2)/4))}
	}{
		\pgfmathparse{#2+((#4-#2)/4)}
	}
	\setcounter{gerdTermID}{1}
	\foreach \pp/\ppl [evaluate=\pp as \x using \pgfmathresult,%#2+((#4-#2)/4),
				  	  evaluate=\pp as \y using #3-(((#5-#3)/(\thegerdNbBodyTerms+1))*\thegerdTermID)]
			in {#6} {	% for each body term
		\node[gerd:term]%, label=$\vpos{\pp}{\ppl}$] 
			(tb\thegerdRuleID_\pp\ppl) at (\x,\y) {$\vpos{\pp}{\ppl}$};% TODO label north west
		\refstepcounter{gerdTermID}
	}


	% compute head terms
	\ifthenelse{\equal{#1}{1}}{
		\pgfmathparse{#2+((#4-#2)/4)}
	}{
		\pgfmathparse{#2+(3*((#4-#2)/4))}
	}
	\setcounter{gerdTermID}{1}
	\foreach \pp/\ppl [evaluate=\pp as \x using \pgfmathresult,
				  evaluate=\pp as \y using #3-(((#5-#3)/(\thegerdNbHeadTerms+1))*\thegerdTermID)]
			in {#7} {	% for each head term
		\node[gerd:term]%, label=$\vpos{\pp}{\ppl}$] 
			(th\thegerdRuleID_\pp\ppl) at (\x,\y) {\bf{$\vpos{\pp}{\ppl}$}};% TODO label north east
		\refstepcounter{gerdTermID}
	}

	% compute edges
	\foreach \ppa/\ppb in {#8} {
		\draw[gerd:edge-norm] (tb\thegerdRuleID_\ppa.east) -- (th\thegerdRuleID_\ppb.west);
		\foreach \te in {#9} {
			\draw[gerd:edge-spec] (tb\thegerdRuleID_\ppa.east) -- (th\thegerdRuleID_\te.west);
		}
	}
}

\newcommand{\gerdUnifA}[4][]{
	\refstepcounter{gerdUnifID}
	\gerdUnif{#1}{#2}{#3}{#4}{$\unifier_{\thegerdUnifID}$}
}

\newcommand{\gerdUnif}[5][]{
	\foreach \th/\tb in {#4} {
		\draw[gerd:edge-unif,#1] (th#2_\th) to node[above]{#5} (tb#3_\tb);
	}
}



%%%% GP

\newenvironment{gp:figure}{
	\begin{tikzpicture}
}{
	\end{tikzpicture}
}

\tikzstyle{gp:node}=[
	gerd:node
]


\tikzstyle{gp:fake}=[
	gp:node,
	gerd:fake
]

\tikzstyle{gp:predpos}=[
	gp:node,
	rectangle,
	minimum size=1mm,
	draw=black
]

\tikzstyle{gp:edge}=[
	gerd:edge
]

\tikzstyle{gp:edge-norm}=[
	gp:edge,
	gerd:edge-norm
]

\tikzstyle{gp:edge-spec}=[
	gp:edge,
	gerd:edge-spec
]

\newcommand{\gpNode}[4]{
	\node[gp:predpos] (#1_#2) at (#3,#4) {$\predpos{#1}{#2}$};
}


\tikzstyle{fake}=[
	inner sep=0mm
]

\tikzstyle{rc:node}=[
]

\tikzstyle{rc:edge}=[
	-,
	draw=black
]

\tikzstyle{rc:complexity-edge}=[
	-,
	thick,
	densely dotted,
	draw
]

\tikzstyle{rc:P-edge}=[
	rc:complexity-edge,
	draw=green!66!black
]

\tikzstyle{rc:NP-edge}=[
	rc:complexity-edge,
	draw=blue!66!black
]

\tikzstyle{rc:ET-edge}=[
	rc:complexity-edge,
	draw=orange!66!black
]

\tikzstyle{rc:ETT-edge}=[
	rc:complexity-edge,
	draw=red!66!black
]

\tikzstyle{rc:complexity-label}=[
]



==> meta/setup.tex <==
% meta/setup.tex

%\geometry{left=1.5cm,right=1cm,marginparwidth=0.5cm,marginparsep=2mm,top=1cm,bottom=1cm}
%\pagenumbering{arabic}
%\pagestyle{fancyplain}

%\hypersetup{
%	urlcolor=blue,
%	linkcolor=black,
%	citecolor=black,
%	colorlinks=true
%}




